Model predictive control with dynamic move blocking

Model Predictive Control (MPC) has proven to be a powerful tool for the control of systems with constraints. Nonetheless, in many applications, a major challenge arises, that is finding the optimal solution within a single sampling instant to apply a receding-horizon policy. In such cases, many suboptimal solutions have been proposed, among which the possibility of "blocking" some moves a-priori. In this paper, we propose a dynamic approach to move blocking, to exploit the solution already available at the previous iteration, and we show not only that such an approach preserves asymptotic stability, but also that the decrease of performance with respect to the ideal solution can be theoretically bounded.

==> Makefile <==
LaTeX=2023-CDC-DMB-MPC

all: compile clean

compile:
	lualatex $(LaTeX).tex
	bibtex $(LaTeX).aux
	lualatex $(LaTeX).tex
	lualatex $(LaTeX).tex

clean: 
	find . -name \*.bbl | xargs rm -f 
	find . -name \*.log | xargs rm -f 
	find . -name \*.lot | xargs rm -f 
	find . -name \*.toc | xargs rm -f 
	find . -name \*.out | xargs rm -f 
	find . -name \*.blg | xargs rm -f 
	find . -name \*.aux | xargs rm -f 
	find . -name \*.ps  | xargs rm -f 
	find . -name \*.dvi | xargs rm -f 
	find . -name \*.snm | xargs rm -f 
	find . -name \*.vrb | xargs rm -f 
	find . -name \*.nav | xargs rm -f
	find . -name \*.vtc | xargs rm -f
	rm -f *.tex~
	rm -f sec/*.tex~
	rm -rf sec/auto
	rm -rf auto
	rm -f *~

view:
	open *.pdf

